Fast, Convexified Stochastic Optimal Open-Loop Control For Linear Systems Using Empirical Characteristic Functions

We consider the problem of stochastic optimal control in the presence of an unknown disturbance. We characterize the disturbance via empirical characteristic functions, and employ a chance constrained approach. By exploiting properties of characteristic functions and underapproximating cumulative distribution functions, we can reformulate a nonconvex problem by a conic, convex under-approximation. This results in extremely fast solutions that are assured to maintain probabilistic constraints. We construct algorithms for optimal open-loop control using piecewise linear approximations of the empirical characteristic function, and demonstrate our approach on two examples.

==> Fast%20Stochastic%20Optimal%20Control%20Using%20Empirical%20Characteristic%20Functions%20(Final)/macrosv1.tex <==
% This file contains a collection of useful macros commonly used by the kinematics and robotics community. 

% Use the command "\input{macrosv1.tex}" to use them in a document. All the macros have been defined so that they can be called without using the math mode delimiter ($) and with xspace. 

%This is version - 1 of this document created on 5th March, 2015.
%-----------------------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------------------

\usepackage{xspace}
\usepackage{amsmath,amssymb,amsfonts}

%-----------------------------------------------------------------------------------------------------

% Generic commands

%% Definition of mathmode bold symbols
\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\mt}[1]{\ensuremath{{#1}}\xspace}

%-----------------------------------------------------------------------------------------------------

% Vector symbols: lower case English characters

\newcommand{\ba}{\ensuremath{\bs a}\xspace}
\newcommand{\bb}{\ensuremath{\bs b}\xspace}
\newcommand{\bc}{\ensuremath{\bs c}\xspace}
\newcommand{\bd}{\ensuremath{\bs d}\xspace}
\newcommand{\be}{\ensuremath{\bs e}\xspace}
\newcommand{\bsf}{\ensuremath{\bs f}\xspace}
\newcommand{\bg}{\ensuremath{\bs g}\xspace}
\newcommand{\bh}{\ensuremath{\bs h}\xspace}
\newcommand{\bi}{\ensuremath{\bs i}\xspace}
\newcommand{\bj}{\ensuremath{\bs j}\xspace}
\newcommand{\bk}{\ensuremath{\bs k}\xspace}
\newcommand{\bl}{\ensuremath{\bs l}\xspace}
\newcommand{\bm}{\ensuremath{\bs m}\xspace}
\newcommand{\bn}{\ensuremath{\bs n}\xspace}
\newcommand{\bo}{\ensuremath{\bs o}\xspace}
\newcommand{\bp}{\ensuremath{\bs p}\xspace}
\newcommand{\bq}{\ensuremath{\bs q}\xspace}
\newcommand{\br}{\ensuremath{\bs r}\xspace}
\newcommand{\bfs}{\ensuremath{\bs s}\xspace}
\newcommand{\bt}{\ensuremath{\bs t}\xspace}
\newcommand{\bu}{\ensuremath{\bs u}\xspace}
\newcommand{\bv}{\ensuremath{\bs v}\xspace}
\newcommand{\bw}{\ensuremath{\bs w}\xspace}
\newcommand{\bx}{\ensuremath{\bs x}\xspace}
\newcommand{\by}{\ensuremath{\bs y}\xspace}
\newcommand{\bz}{\ensuremath{\bs z}\xspace}

% Matrix symbols: upper case English characters

\newcommand{\bA}{\ensuremath{\bs A}\xspace}
\newcommand{\bB}{\ensuremath{\bs B}\xspace}
\newcommand{\bC}{\ensuremath{\bs C}\xspace}
\newcommand{\bD}{\ensuremath{\bs D}\xspace}
\newcommand{\bE}{\ensuremath{\bs E}\xspace}
\newcommand{\bF}{\ensuremath{\bs F}\xspace}
\newcommand{\bG}{\ensuremath{\bs G}\xspace}
\newcommand{\bH}{\ensuremath{\bs H}\xspace}
\newcommand{\bI}{\ensuremath{\bs I}\xspace}
\newcommand{\bJ}{\ensuremath{\bs J}\xspace}
\newcommand{\bK}{\ensuremath{\bs K}\xspace}
\newcommand{\bL}{\ensuremath{\bs L}\xspace}
\newcommand{\bM}{\ensuremath{\bs M}\xspace}
\newcommand{\bN}{\ensuremath{\bs N}\xspace}
\newcommand{\bO}{\ensuremath{\bs O}\xspace}
\newcommand{\bP}{\ensuremath{\bs P}\xspace}
\newcommand{\bQ}{\ensuremath{\bs Q}\xspace}
\newcommand{\bR}{\ensuremath{\bs R}\xspace}
\newcommand{\bS}{\ensuremath{\bs S}\xspace}
\newcommand{\bT}{\ensuremath{\bs T}\xspace}
\newcommand{\bU}{\ensuremath{\bs U}\xspace}
\newcommand{\bV}{\ensuremath{\bs V}\xspace}
\newcommand{\bW}{\ensuremath{\bs W}\xspace}
\newcommand{\bX}{\ensuremath{\bs X}\xspace}
\newcommand{\bY}{\ensuremath{\bs Y}\xspace}
\newcommand{\bZ}{\ensuremath{\bs Z}\xspace}

% Greek letters

%% Mathmode greek symbols, lower case
\newcommand{\alp}{\ensuremath{\alpha}\xspace}
\newcommand{\bet}{\ensuremath{\beta}\xspace}
\newcommand{\gm}{\ensuremath{\gamma}\xspace}
\newcommand{\del}{\ensuremath{\delta}\xspace}
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}
\newcommand{\veps}{\ensuremath{\varepsilon}\xspace}
\newcommand{\zet}{\ensuremath{\zeta}\xspace}
\newcommand{\et}{\ensuremath{\eta}\xspace}
\newcommand{\tht}{\ensuremath{\theta}\xspace}
\newcommand{\vth}{\ensuremath{\vartheta}\xspace}
\newcommand{\iot}{\ensuremath{\iota}\xspace}
\newcommand{\kap}{\ensuremath{\kappa}\xspace}
\newcommand{\vkap}{\ensuremath{\varkappa}\xspace}
\newcommand{\lam}{\ensuremath{\lambda}\xspace}
\newcommand{\mmu}{\ensuremath{\mu}\xspace}
\newcommand{\mnu}{\ensuremath{\nu}\xspace}
\newcommand{\mxi}{\ensuremath{\xi}\xspace}
\newcommand{\omic}{\ensuremath{\omicron}\xspace}
\newcommand{\mpi}{\ensuremath{\pi}\xspace}
\newcommand{\vpi}{\ensuremath{\varpi}\xspace}
\newcommand{\mrho}{\ensuremath{\rho}\xspace}
\newcommand{\vrho}{\ensuremath{\varrho}\xspace}
\newcommand{\sig}{\ensuremath{\sigma}\xspace}
\newcommand{\vsig}{\ensuremath{\varsigma}\xspace}
\newcommand{\mtau}{\ensuremath{\tau}\xspace}
\newcommand{\ups}{\ensuremath{\upsilon}\xspace}
\newcommand{\ph}{\ensuremath{\phi}\xspace}
\newcommand{\vph}{\ensuremath{\varphi}\xspace}
\newcommand{\mchi}{\ensuremath{\chi}\xspace}
\newcommand{\mpsi}{\ensuremath{\psi}\xspace}
\newcommand{\om}{\ensuremath{\omega}\xspace}

%% Mathmode bold Greek symbols, lower case
\newcommand{\balp}{\ensuremath{\bs \alpha}\xspace}
\newcommand{\bbet}{\ensuremath{\bs \beta}\xspace}
\newcommand{\bgamma}{\ensuremath{\bs \gamma}\xspace}
\newcommand{\bdel}{\ensuremath{\bs \delta}\xspace}
\newcommand{\beps}{\ensuremath{\bs \epsilon}\xspace}
\newcommand{\bveps}{\ensuremath{\bs \varepsilon}\xspace}
\newcommand{\bzet}{\ensuremath{\bs \zeta}\xspace}
\newcommand{\bfeta}{\ensuremath{\bs \eta}\xspace}
\newcommand{\bth}{\ensuremath{\bs \theta}\xspace}
\newcommand{\bvth}{\ensuremath{\bs \vartheta}\xspace}
\newcommand{\biot}{\ensuremath{\bs \iota}\xspace}
\newcommand{\bkap}{\ensuremath{\bs \kappa}\xspace}
\newcommand{\bvkap}{\ensuremath{\bs \varkappa}\xspace}
\newcommand{\blam}{\ensuremath{\bs \lambda}\xspace}
\newcommand{\bmu}{\ensuremath{\bs \mu}\xspace}
\newcommand{\bnu}{\ensuremath{\bs \nu}\xspace}
\newcommand{\bxi}{\ensuremath{\bs \xi}\xspace}
\newcommand{\bomic}{\ensuremath{\bs \omicron}\xspace}
\newcommand{\bpi}{\ensuremath{\bs \pi}\xspace}
\newcommand{\bvpi}{\ensuremath{\bs \varpi}\xspace}
\newcommand{\brho}{\ensuremath{\bs \rho}\xspace}
\newcommand{\bvrho}{\ensuremath{\bs \varrho}\xspace}
\newcommand{\bsig}{\ensuremath{\bs \sigma}\xspace}
\newcommand{\bvsig}{\ensuremath{\bs \varsigma}\xspace}
\newcommand{\btau}{\ensuremath{\bs \tau}\xspace}
\newcommand{\bups}{\ensuremath{\bs \upsilon}\xspace}
\newcommand{\bphi}{\ensuremath{\bs \phi}\xspace}
\newcommand{\nvph}{\ensuremath{\bs \varphi}\xspace}
\newcommand{\bch}{\ensuremath{\bs \chi}\xspace}
\newcommand{\bpsi}{\ensuremath{\bs \psi}\xspace}
\newcommand{\bom}{\ensuremath{\bs \omega}\xspace}

%% Mathmode Greek symbols,upper case
\newcommand{\Gm}{\ensuremath{\Gamma}\xspace}
\newcommand{\Del}{\ensuremath{\Delta}\xspace}
\newcommand{\Th}{\ensuremath{\Theta}\xspace}
\newcommand{\Lam}{\ensuremath{\Lambda}\xspace}
\newcommand{\mXi}{\ensuremath{\Xi}\xspace}
\newcommand{\mPi}{\ensuremath{\Pi}\xspace}
\newcommand{\Sig}{\ensuremath{\Sigma}\xspace}
\newcommand{\Ups}{\ensuremath{\Upsilon}\xspace}
\newcommand{\Ph}{\ensuremath{\Phi}\xspace}
\newcommand{\Ps}{\ensuremath{\Psi}\xspace}
\newcommand{\Om}{\ensuremath{\Omega}\xspace}

%% Mathmode bold Greek symbols, upper case
\newcommand{\bGm}{\ensuremath{\bs \Gamma}\xspace}
\newcommand{\bDel}{\ensuremath{\bs \Delta}\xspace}
\newcommand{\bTh}{\ensuremath{\bs \Theta}\xspace}
\newcommand{\bLam}{\ensuremath{\bs \Lambda}\xspace}
\newcommand{\bXi}{\ensuremath{\bs \Xi}\xspace}
\newcommand{\bPi}{\ensuremath{\bs \Pi}\xspace}
\newcommand{\bSig}{\ensuremath{\bs \Sigma}\xspace}
\newcommand{\bUps}{\ensuremath{\bs \Upsilon}\xspace}
\newcommand{\bPhi}{\ensuremath{\bs \Phi}\xspace}
\newcommand{\bPsi}{\ensuremath{\bs \Psi}\xspace}
\newcommand{\bOm}{\ensuremath{\bs{\Omega}}\xspace}

% Vector/matrix "zero"
\newcommand{\bzero}{\ensuremath{\bs{0}}\xspace}

% Half
\newcommand{\half}{\ensuremath{\frac{1}{2}}\xspace}

%-----------------------------------------------------------------------------------------------------

%  Spaces symbols

\newcommand{\C}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\Cn}{\ensuremath{\mathbb{C}^n}\xspace}
\newcommand{\D}{\ensuremath{\mathbb{D}}\xspace}
\newcommand{\Dn}{\ensuremath{\mathbb{D}^n}\xspace}
\renewcommand{\Re}{\ensuremath{\mathbb{R}}\xspace} % latex2e
\newcommand{\Rn}{\ensuremath{\mathbb{R}^n}\xspace}
%\newcommand{\se}{\ensuremath{se(3)}\xspace}
%\newcommand{\ses}{\ensuremath{se^*(3)}\xspace}
%\newcommand{\SE}{\ensuremath{\mathbb{SE}(3)}\xspace}
%\newcommand{\so}{\ensuremath{so(3)}\xspace}
%\newcommand{\SO}{\ensuremath{\mathbb{SO}(3)}\xspace}


%% Notations for the configuration space
\newcommand{\conf}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\dimc}{\ensuremath{\textrm{dim(}\mathcal{C}}\textrm{)}\xspace}

%-----------------------------------------------------------------------------------------------------
% Jacobian matrices

%% Constraint Jacobian matrices
\newcommand{\jetaq}{\ensuremath{{\boldsymbol J}_{\bfeta\bq}}\xspace}
\newcommand{\jetath}{\ensuremath{{\bs J}_{\bfeta\bth}}\xspace}
\newcommand{\jetaphi}{\ensuremath{{\bs J}_{\bfeta\bphi}}\xspace}
\newcommand{\jetagamma}{\ensuremath{{\bs J}_{\bfeta\bgamma}}\xspace}
\newcommand{\jetapsi}{\ensuremath{{\bs J}_{\bfeta\bpsi}}\xspace}
\newcommand{\jphith}{\ensuremath{{\bs J}_{\bphi\bth}}\xspace}
\newcommand{\jpsith}{\ensuremath{{\bs J}_{\bpsi\bth}}\xspace}
\newcommand{\jgammath}{\ensuremath{{\bs J}_{\bgamma\bth}}\xspace}

\newcommand{\jqth}{\ensuremath{{\boldsymbol{J}}_{\bq\bth}}\xspace}
\newcommand{\jpq}{\ensuremath{{\boldsymbol{J}}_{\bp\bq}}\xspace}

\newcommand{\jpcth}{\ensuremath{\boldsymbol{J}_{\pc\bth}\xspace}}
\newcommand{\jpcphi}{\ensuremath{\boldsymbol{J}_{\pc\bphi}\xspace}}
\newcommand{\jpcq}{\ensuremath{\boldsymbol{J}_{\pc\bq}\xspace}}

\newcommand{\jfth}{\ensuremath{\boldsymbol{J}_{\bs{f}\bth}\xspace}}
\newcommand{\jfpsi}{\ensuremath{\boldsymbol{J}_{\bs{f}\bpsi}\xspace}}
\newcommand{\jfrts}{\ensuremath{\boldsymbol{J}_{\bs{f}\bs{r}_{ts}}\xspace}}
\newcommand{\jfpc}{\ensuremath{\boldsymbol{J}_{\bs{f}\bp_c}\xspace}}

\newcommand{\jpth}{\ensuremath{\boldsymbol{J}_{\boldsymbol{p\theta}}\xspace}}
\newcommand{\jpphi}{\ensuremath{\boldsymbol{J}_{\boldsymbol{p\phi}}\xspace}}

%% Angular velocity related
\newcommand{\jom}{\ensuremath{{\bs J}_{\bom}}\xspace}
\newcommand{\jomc}[1]{\ensuremath{{\boldsymbol J}_{\boldsymbol{\omega}_{c_#1}}}\xspace}
\newcommand{\jomth}{\ensuremath{{\bs J}_{\bom\bth}}\xspace}
\newcommand{\jomphi}{\ensuremath{{\bs J}_{\bom\bphi}}\xspace}
\newcommand{\jomeq}{\ensuremath{{\bs J}_{\bom}^{eq}}\xspace}
\newcommand{\jweq}{\ensuremath{{\bs J}_{\bs{w}}^{eq}}\xspace}

%% Linear velocity related
\newcommand{\jv}{\ensuremath{{\bs J}_{\bs v}}\xspace}
\newcommand{\jvp}{\ensuremath{{\bs J}_{{\bs v}{\bs p}}}\xspace}
\newcommand{\jvth}{\ensuremath{{\bs J}_{\bv\bth}}\xspace}
\newcommand{\jvphi}{\ensuremath{{\bs J}_{\bv\bphi}}\xspace}
\newcommand{\jveq}{\ensuremath{{\bs J}_{\bv}^{eq}}\xspace}
\newcommand{\jc}{\ensuremath{{\bs J}_{\bs c}}\xspace}
\newcommand{\jvpc}[1]{\ensuremath{\boldsymbol{J}_{{\boldsymbol{v}_{\boldsymbol{p}_{c_#1}}}}\xspace}}
\newcommand{\jcp}{\ensuremath{\bs{J}_{\bs{c}{\bp}}}\xspace}

%-----------------------------------------------------------------------------------------------------
% Kinematics

\newcommand{\rot}[2]{\ensuremath{{}^{#1}_{#2}{\boldsymbol{R}}}\xspace}%rotation matrix
\newcommand{\tran}[2]{\ensuremath{{}^{#1}_{#2}{\boldsymbol{T}}}\xspace}
\newcommand{\frm}[1]{\ensuremath{\{#1\}}\xspace} % frame number
\newcommand{\pc}{\ensuremath{\boldsymbol{p}_c}\xspace}
\newcommand{\pci}[1]{\ensuremath{\bs{p}_{\boldsymbol{c}_{i}}}\xspace}

%% Velocities
\newcommand{\vp}{\ensuremath{\bs{v}_{\boldsymbol{p}}}\xspace} % place with velocity commands
\newcommand{\vpc}[1]{\ensuremath{\bs{v}_{\boldsymbol{p}_{c_#1}}}\xspace}

%% Derivatives
\newcommand{\xd}{\ensuremath{\dot{x}}\xspace}
\newcommand{\xdd}{\ensuremath{\ddot{x}}\xspace}
\newcommand{\bqd}{\ensuremath{\dot{\boldsymbol{q}}}\xspace}
\newcommand{\bqdd}{\ensuremath{\ddot{\boldsymbol{q}}}\xspace}
\newcommand{\pcd}{\ensuremath{\dot{\boldsymbol{p}_c}}\xspace}

\newcommand{\bthd}{\ensuremath{\dot{\bs{\theta}}}\xspace}
\newcommand{\bthdd}{\ensuremath{\ddot{\bth}}\xspace}
\newcommand{\alphad}{\ensuremath{\dot \alpha}\xspace}
\newcommand{\psid}{\ensuremath{\dot{\psi}}\xspace}
\newcommand{\psidd}{\ensuremath{\ddot{\psi}}\xspace}
\newcommand{\phid}{\ensuremath{\dot{\phi}}\xspace}
\newcommand{\bPhid}{\ensuremath{\dot{\bs{\Phi}}}\xspace}
\newcommand{\bphid}{\ensuremath{\dot{\bs{\phi}}}\xspace}
\newcommand{\bpsid}{\ensuremath{\dot{\bs{\psi}}}\xspace}

%-----------------------------------------------------------------------------------------------------.
% Dynamics

\newcommand{\bMth}{\ensuremath{\bs{M_\theta}}\xspace}
\newcommand{\bCth}{\ensuremath{\bs{C_\theta}}\xspace}
\newcommand{\bGth}{\ensuremath{\bs{G_\theta}}\xspace}

\newcommand{\bin}{\ensuremath{\bs{I}_n}\xspace}
\newcommand{\Ith}{\ensuremath{I(\theta)}\xspace}

\newcommand{\bkp}{\ensuremath{\boldsymbol{K}_p}\xspace}
\newcommand{\bkv}{\ensuremath{\boldsymbol{K}_v}\xspace}

\newcommand{\bQnc}{\ensuremath{\boldsymbol{Q}^{nc}}\xspace}

%-----------------------------------------------------------------------------------------------------.
% Manipulators

\newcommand{\rrs}{\ensuremath{3}-\underline{R}RS\xspace}
\newcommand{\rps}{\ensuremath{3}-R\underline{P}S\xspace}
\newcommand{\upu}{\ensuremath{3}-U\underline{P}U\xspace}
%\newcommand{\map}{\mbox{MaPaMan}\xspace}
%\newcommand{\mapI}{\mbox{MaPaMan-I}\xspace}
%\newcommand{\mapII}{\mbox{MaPaMan-II}\xspace}
\newcommand{\rrr}{\ensuremath{3}-\underline{R}RR\xspace}
\newcommand{\rpr}{\ensuremath{3}-R\underline{P}R\xspace}

%-----------------------------------------------------------------------------------------------------

% Math Symbols

\renewcommand{\iff}{\ensuremath{\mathit{iff}}\xspace}
%\newtheorem{thm}{Theorem}[section]
%\newcommand{\implies}{\ensuremath{\Rightarrow \;}\xspace}
\def\QED{\ensuremath{\rule[0pt]{1.5ex}{1.5ex}}\xspace}
\def\proof{\noindent\hspace{2em}{\em Proof: }}
\def\endproof{\hspace*{\fill}~\QED\par\endtrivlist\unskip}
%\newcommand{\mathe}{\begin{verbatim}Mathematica\end{verbatim}\xspace}
%\newcommand{\define}{\ensuremath{\stackrel{\Delta}{=}}\xspace}
\newcommand{\elim}[1]{\ensuremath{\stackrel{\times #1}{\longrightarrow}}\xspace}

%% Operations
\newcommand{\adj}{\text{adj}}
\newcommand{\trace}{\text{tr}}

%%% Norm
\newcommand{\norm}[1]{\ensuremath{\| #1\|}\xspace}
\newcommand{\normd}[1]{\ensuremath{\| #1\|_d}\xspace}

%%% Partial derivative
\newcommand{\pd}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}\xspace}
\newcommand{\dpd}[2]{\ensuremath{\dfrac{\partial #1}{\partial #2}}\xspace}

%%% Total derivative
\newcommand{\td}[2]{\ensuremath{\frac{d #1}{d #2}}\xspace}
\newcommand{\dtotder}[2]{\ensuremath{\dfrac{d #1}{d #2}}\xspace}

%%% Partial second derivative
\newcommand{\pdd}[2]{\ensuremath{\frac{\partial^2 #1}{\partial #2^2}}\xspace}

%%% Total second derivative
\newcommand{\tdd}[2]{\ensuremath{\frac{d^2 #1}{d #2^2}}\xspace}
\newcommand{\dsecder}[2]{\ensuremath{\dfrac{\partial^2 #1}{\partial #2^2}}\xspace}

%%% Scalar tripple product
\newcommand{\trip}[3]{\ensuremath{\left[#1, #2, #3\right]\xspace}}

%% Rank symbols
%\newcommand{\rank}[1]{\ensuremath{\mathrm{rank}\left(#1\right)}\xspace}

%-----------------------------------------------------------------------------------------------------

% Generic words

\newcommand{\dof}{degree-of-freedom\xspace}
\newcommand{\dofs}{degrees-of-freedom\xspace}
\newcommand{\rb}{rigid-body\xspace}
\newcommand{\rbm}{rigid-body motion\xspace}

%-----------------------------------------------------------------------------------------------------


==> macrosv1.tex <==
% This file contains a collection of useful macros commonly used by the kinematics and robotics community. 

% Use the command "\input{macrosv1.tex}" to use them in a document. All the macros have been defined so that they can be called without using the math mode delimiter ($) and with xspace. 

%This is version - 1 of this document created on 5th March, 2015.
%-----------------------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------------------

\usepackage{xspace}
\usepackage{amsmath,amssymb,amsfonts}

%-----------------------------------------------------------------------------------------------------

% Generic commands

%% Definition of mathmode bold symbols
\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\mt}[1]{\ensuremath{{#1}}\xspace}

%-----------------------------------------------------------------------------------------------------

% Vector symbols: lower case English characters

\newcommand{\ba}{\ensuremath{\bs a}\xspace}
\newcommand{\bb}{\ensuremath{\bs b}\xspace}
\newcommand{\bc}{\ensuremath{\bs c}\xspace}
\newcommand{\bd}{\ensuremath{\bs d}\xspace}
\newcommand{\be}{\ensuremath{\bs e}\xspace}
\newcommand{\bsf}{\ensuremath{\bs f}\xspace}
\newcommand{\bg}{\ensuremath{\bs g}\xspace}
\newcommand{\bh}{\ensuremath{\bs h}\xspace}
\newcommand{\bi}{\ensuremath{\bs i}\xspace}
\newcommand{\bj}{\ensuremath{\bs j}\xspace}
\newcommand{\bk}{\ensuremath{\bs k}\xspace}
\newcommand{\bl}{\ensuremath{\bs l}\xspace}
\newcommand{\bm}{\ensuremath{\bs m}\xspace}
\newcommand{\bn}{\ensuremath{\bs n}\xspace}
\newcommand{\bo}{\ensuremath{\bs o}\xspace}
\newcommand{\bp}{\ensuremath{\bs p}\xspace}
\newcommand{\bq}{\ensuremath{\bs q}\xspace}
\newcommand{\br}{\ensuremath{\bs r}\xspace}
\newcommand{\bfs}{\ensuremath{\bs s}\xspace}
\newcommand{\bt}{\ensuremath{\bs t}\xspace}
\newcommand{\bu}{\ensuremath{\bs u}\xspace}
\newcommand{\bv}{\ensuremath{\bs v}\xspace}
\newcommand{\bw}{\ensuremath{\bs w}\xspace}
\newcommand{\bx}{\ensuremath{\bs x}\xspace}
\newcommand{\by}{\ensuremath{\bs y}\xspace}
\newcommand{\bz}{\ensuremath{\bs z}\xspace}

% Matrix symbols: upper case English characters

\newcommand{\bA}{\ensuremath{\bs A}\xspace}
\newcommand{\bB}{\ensuremath{\bs B}\xspace}
\newcommand{\bC}{\ensuremath{\bs C}\xspace}
\newcommand{\bD}{\ensuremath{\bs D}\xspace}
\newcommand{\bE}{\ensuremath{\bs E}\xspace}
\newcommand{\bF}{\ensuremath{\bs F}\xspace}
\newcommand{\bG}{\ensuremath{\bs G}\xspace}
\newcommand{\bH}{\ensuremath{\bs H}\xspace}
\newcommand{\bI}{\ensuremath{\bs I}\xspace}
\newcommand{\bJ}{\ensuremath{\bs J}\xspace}
\newcommand{\bK}{\ensuremath{\bs K}\xspace}
\newcommand{\bL}{\ensuremath{\bs L}\xspace}
\newcommand{\bM}{\ensuremath{\bs M}\xspace}
\newcommand{\bN}{\ensuremath{\bs N}\xspace}
\newcommand{\bO}{\ensuremath{\bs O}\xspace}
\newcommand{\bP}{\ensuremath{\bs P}\xspace}
\newcommand{\bQ}{\ensuremath{\bs Q}\xspace}
\newcommand{\bR}{\ensuremath{\bs R}\xspace}
\newcommand{\bS}{\ensuremath{\bs S}\xspace}
\newcommand{\bT}{\ensuremath{\bs T}\xspace}
\newcommand{\bU}{\ensuremath{\bs U}\xspace}
\newcommand{\bV}{\ensuremath{\bs V}\xspace}
\newcommand{\bW}{\ensuremath{\bs W}\xspace}
\newcommand{\bX}{\ensuremath{\bs X}\xspace}
\newcommand{\bY}{\ensuremath{\bs Y}\xspace}
\newcommand{\bZ}{\ensuremath{\bs Z}\xspace}

% Greek letters

%% Mathmode greek symbols, lower case
\newcommand{\alp}{\ensuremath{\alpha}\xspace}
\newcommand{\bet}{\ensuremath{\beta}\xspace}
\newcommand{\gm}{\ensuremath{\gamma}\xspace}
\newcommand{\del}{\ensuremath{\delta}\xspace}
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}
\newcommand{\veps}{\ensuremath{\varepsilon}\xspace}
\newcommand{\zet}{\ensuremath{\zeta}\xspace}
\newcommand{\et}{\ensuremath{\eta}\xspace}
\newcommand{\tht}{\ensuremath{\theta}\xspace}
\newcommand{\vth}{\ensuremath{\vartheta}\xspace}
\newcommand{\iot}{\ensuremath{\iota}\xspace}
\newcommand{\kap}{\ensuremath{\kappa}\xspace}
\newcommand{\vkap}{\ensuremath{\varkappa}\xspace}
\newcommand{\lam}{\ensuremath{\lambda}\xspace}
\newcommand{\mmu}{\ensuremath{\mu}\xspace}
\newcommand{\mnu}{\ensuremath{\nu}\xspace}
\newcommand{\mxi}{\ensuremath{\xi}\xspace}
\newcommand{\omic}{\ensuremath{\omicron}\xspace}
\newcommand{\mpi}{\ensuremath{\pi}\xspace}
\newcommand{\vpi}{\ensuremath{\varpi}\xspace}
\newcommand{\mrho}{\ensuremath{\rho}\xspace}
\newcommand{\vrho}{\ensuremath{\varrho}\xspace}
\newcommand{\sig}{\ensuremath{\sigma}\xspace}
\newcommand{\vsig}{\ensuremath{\varsigma}\xspace}
\newcommand{\mtau}{\ensuremath{\tau}\xspace}
\newcommand{\ups}{\ensuremath{\upsilon}\xspace}
\newcommand{\ph}{\ensuremath{\phi}\xspace}
\newcommand{\vph}{\ensuremath{\varphi}\xspace}
\newcommand{\mchi}{\ensuremath{\chi}\xspace}
\newcommand{\mpsi}{\ensuremath{\psi}\xspace}
\newcommand{\om}{\ensuremath{\omega}\xspace}

%% Mathmode bold Greek symbols, lower case
\newcommand{\balp}{\ensuremath{\bs \alpha}\xspace}
\newcommand{\bbet}{\ensuremath{\bs \beta}\xspace}
\newcommand{\bgamma}{\ensuremath{\bs \gamma}\xspace}
\newcommand{\bdel}{\ensuremath{\bs \delta}\xspace}
\newcommand{\beps}{\ensuremath{\bs \epsilon}\xspace}
\newcommand{\bveps}{\ensuremath{\bs \varepsilon}\xspace}
\newcommand{\bzet}{\ensuremath{\bs \zeta}\xspace}
\newcommand{\bfeta}{\ensuremath{\bs \eta}\xspace}
\newcommand{\bth}{\ensuremath{\bs \theta}\xspace}
\newcommand{\bvth}{\ensuremath{\bs \vartheta}\xspace}
\newcommand{\biot}{\ensuremath{\bs \iota}\xspace}
\newcommand{\bkap}{\ensuremath{\bs \kappa}\xspace}
\newcommand{\bvkap}{\ensuremath{\bs \varkappa}\xspace}
\newcommand{\blam}{\ensuremath{\bs \lambda}\xspace}
\newcommand{\bmu}{\ensuremath{\bs \mu}\xspace}
\newcommand{\bnu}{\ensuremath{\bs \nu}\xspace}
\newcommand{\bxi}{\ensuremath{\bs \xi}\xspace}
\newcommand{\bomic}{\ensuremath{\bs \omicron}\xspace}
\newcommand{\bpi}{\ensuremath{\bs \pi}\xspace}
\newcommand{\bvpi}{\ensuremath{\bs \varpi}\xspace}
\newcommand{\brho}{\ensuremath{\bs \rho}\xspace}
\newcommand{\bvrho}{\ensuremath{\bs \varrho}\xspace}
\newcommand{\bsig}{\ensuremath{\bs \sigma}\xspace}
\newcommand{\bvsig}{\ensuremath{\bs \varsigma}\xspace}
\newcommand{\btau}{\ensuremath{\bs \tau}\xspace}
\newcommand{\bups}{\ensuremath{\bs \upsilon}\xspace}
\newcommand{\bphi}{\ensuremath{\bs \phi}\xspace}
\newcommand{\nvph}{\ensuremath{\bs \varphi}\xspace}
\newcommand{\bch}{\ensuremath{\bs \chi}\xspace}
\newcommand{\bpsi}{\ensuremath{\bs \psi}\xspace}
\newcommand{\bom}{\ensuremath{\bs \omega}\xspace}

%% Mathmode Greek symbols,upper case
\newcommand{\Gm}{\ensuremath{\Gamma}\xspace}
\newcommand{\Del}{\ensuremath{\Delta}\xspace}
\newcommand{\Th}{\ensuremath{\Theta}\xspace}
\newcommand{\Lam}{\ensuremath{\Lambda}\xspace}
\newcommand{\mXi}{\ensuremath{\Xi}\xspace}
\newcommand{\mPi}{\ensuremath{\Pi}\xspace}
\newcommand{\Sig}{\ensuremath{\Sigma}\xspace}
\newcommand{\Ups}{\ensuremath{\Upsilon}\xspace}
\newcommand{\Ph}{\ensuremath{\Phi}\xspace}
\newcommand{\Ps}{\ensuremath{\Psi}\xspace}
\newcommand{\Om}{\ensuremath{\Omega}\xspace}

%% Mathmode bold Greek symbols, upper case
\newcommand{\bGm}{\ensuremath{\bs \Gamma}\xspace}
\newcommand{\bDel}{\ensuremath{\bs \Delta}\xspace}
\newcommand{\bTh}{\ensuremath{\bs \Theta}\xspace}
\newcommand{\bLam}{\ensuremath{\bs \Lambda}\xspace}
\newcommand{\bXi}{\ensuremath{\bs \Xi}\xspace}
\newcommand{\bPi}{\ensuremath{\bs \Pi}\xspace}
\newcommand{\bSig}{\ensuremath{\bs \Sigma}\xspace}
\newcommand{\bUps}{\ensuremath{\bs \Upsilon}\xspace}
\newcommand{\bPhi}{\ensuremath{\bs \Phi}\xspace}
\newcommand{\bPsi}{\ensuremath{\bs \Psi}\xspace}
\newcommand{\bOm}{\ensuremath{\bs{\Omega}}\xspace}

% Vector/matrix "zero"
\newcommand{\bzero}{\ensuremath{\bs{0}}\xspace}

% Half
\newcommand{\half}{\ensuremath{\frac{1}{2}}\xspace}

%-----------------------------------------------------------------------------------------------------

%  Spaces symbols

\newcommand{\C}{\ensuremath{\mathbb{C}}\xspace}
\newcommand{\Cn}{\ensuremath{\mathbb{C}^n}\xspace}
\newcommand{\D}{\ensuremath{\mathbb{D}}\xspace}
\newcommand{\Dn}{\ensuremath{\mathbb{D}^n}\xspace}
\renewcommand{\Re}{\ensuremath{\mathbb{R}}\xspace} % latex2e
\newcommand{\Rn}{\ensuremath{\mathbb{R}^n}\xspace}
%\newcommand{\se}{\ensuremath{se(3)}\xspace}
%\newcommand{\ses}{\ensuremath{se^*(3)}\xspace}
%\newcommand{\SE}{\ensuremath{\mathbb{SE}(3)}\xspace}
%\newcommand{\so}{\ensuremath{so(3)}\xspace}
%\newcommand{\SO}{\ensuremath{\mathbb{SO}(3)}\xspace}


%% Notations for the configuration space
\newcommand{\conf}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\dimc}{\ensuremath{\textrm{dim(}\mathcal{C}}\textrm{)}\xspace}

%-----------------------------------------------------------------------------------------------------
% Jacobian matrices

%% Constraint Jacobian matrices
\newcommand{\jetaq}{\ensuremath{{\boldsymbol J}_{\bfeta\bq}}\xspace}
\newcommand{\jetath}{\ensuremath{{\bs J}_{\bfeta\bth}}\xspace}
\newcommand{\jetaphi}{\ensuremath{{\bs J}_{\bfeta\bphi}}\xspace}
\newcommand{\jetagamma}{\ensuremath{{\bs J}_{\bfeta\bgamma}}\xspace}
\newcommand{\jetapsi}{\ensuremath{{\bs J}_{\bfeta\bpsi}}\xspace}
\newcommand{\jphith}{\ensuremath{{\bs J}_{\bphi\bth}}\xspace}
\newcommand{\jpsith}{\ensuremath{{\bs J}_{\bpsi\bth}}\xspace}
\newcommand{\jgammath}{\ensuremath{{\bs J}_{\bgamma\bth}}\xspace}

\newcommand{\jqth}{\ensuremath{{\boldsymbol{J}}_{\bq\bth}}\xspace}
\newcommand{\jpq}{\ensuremath{{\boldsymbol{J}}_{\bp\bq}}\xspace}

\newcommand{\jpcth}{\ensuremath{\boldsymbol{J}_{\pc\bth}\xspace}}
\newcommand{\jpcphi}{\ensuremath{\boldsymbol{J}_{\pc\bphi}\xspace}}
\newcommand{\jpcq}{\ensuremath{\boldsymbol{J}_{\pc\bq}\xspace}}

\newcommand{\jfth}{\ensuremath{\boldsymbol{J}_{\bs{f}\bth}\xspace}}
\newcommand{\jfpsi}{\ensuremath{\boldsymbol{J}_{\bs{f}\bpsi}\xspace}}
\newcommand{\jfrts}{\ensuremath{\boldsymbol{J}_{\bs{f}\bs{r}_{ts}}\xspace}}
\newcommand{\jfpc}{\ensuremath{\boldsymbol{J}_{\bs{f}\bp_c}\xspace}}

\newcommand{\jpth}{\ensuremath{\boldsymbol{J}_{\boldsymbol{p\theta}}\xspace}}
\newcommand{\jpphi}{\ensuremath{\boldsymbol{J}_{\boldsymbol{p\phi}}\xspace}}

%% Angular velocity related
\newcommand{\jom}{\ensuremath{{\bs J}_{\bom}}\xspace}
\newcommand{\jomc}[1]{\ensuremath{{\boldsymbol J}_{\boldsymbol{\omega}_{c_#1}}}\xspace}
\newcommand{\jomth}{\ensuremath{{\bs J}_{\bom\bth}}\xspace}
\newcommand{\jomphi}{\ensuremath{{\bs J}_{\bom\bphi}}\xspace}
\newcommand{\jomeq}{\ensuremath{{\bs J}_{\bom}^{eq}}\xspace}
\newcommand{\jweq}{\ensuremath{{\bs J}_{\bs{w}}^{eq}}\xspace}

%% Linear velocity related
\newcommand{\jv}{\ensuremath{{\bs J}_{\bs v}}\xspace}
\newcommand{\jvp}{\ensuremath{{\bs J}_{{\bs v}{\bs p}}}\xspace}
\newcommand{\jvth}{\ensuremath{{\bs J}_{\bv\bth}}\xspace}
\newcommand{\jvphi}{\ensuremath{{\bs J}_{\bv\bphi}}\xspace}
\newcommand{\jveq}{\ensuremath{{\bs J}_{\bv}^{eq}}\xspace}
\newcommand{\jc}{\ensuremath{{\bs J}_{\bs c}}\xspace}
\newcommand{\jvpc}[1]{\ensuremath{\boldsymbol{J}_{{\boldsymbol{v}_{\boldsymbol{p}_{c_#1}}}}\xspace}}
\newcommand{\jcp}{\ensuremath{\bs{J}_{\bs{c}{\bp}}}\xspace}

%-----------------------------------------------------------------------------------------------------
% Kinematics

\newcommand{\rot}[2]{\ensuremath{{}^{#1}_{#2}{\boldsymbol{R}}}\xspace}%rotation matrix
\newcommand{\tran}[2]{\ensuremath{{}^{#1}_{#2}{\boldsymbol{T}}}\xspace}
\newcommand{\frm}[1]{\ensuremath{\{#1\}}\xspace} % frame number
\newcommand{\pc}{\ensuremath{\boldsymbol{p}_c}\xspace}
\newcommand{\pci}[1]{\ensuremath{\bs{p}_{\boldsymbol{c}_{i}}}\xspace}

%% Velocities
\newcommand{\vp}{\ensuremath{\bs{v}_{\boldsymbol{p}}}\xspace} % place with velocity commands
\newcommand{\vpc}[1]{\ensuremath{\bs{v}_{\boldsymbol{p}_{c_#1}}}\xspace}

%% Derivatives
\newcommand{\xd}{\ensuremath{\dot{x}}\xspace}
\newcommand{\xdd}{\ensuremath{\ddot{x}}\xspace}
\newcommand{\bqd}{\ensuremath{\dot{\boldsymbol{q}}}\xspace}
\newcommand{\bqdd}{\ensuremath{\ddot{\boldsymbol{q}}}\xspace}
\newcommand{\pcd}{\ensuremath{\dot{\boldsymbol{p}_c}}\xspace}

\newcommand{\bthd}{\ensuremath{\dot{\bs{\theta}}}\xspace}
\newcommand{\bthdd}{\ensuremath{\ddot{\bth}}\xspace}
\newcommand{\alphad}{\ensuremath{\dot \alpha}\xspace}
\newcommand{\psid}{\ensuremath{\dot{\psi}}\xspace}
\newcommand{\psidd}{\ensuremath{\ddot{\psi}}\xspace}
\newcommand{\phid}{\ensuremath{\dot{\phi}}\xspace}
\newcommand{\bPhid}{\ensuremath{\dot{\bs{\Phi}}}\xspace}
\newcommand{\bphid}{\ensuremath{\dot{\bs{\phi}}}\xspace}
\newcommand{\bpsid}{\ensuremath{\dot{\bs{\psi}}}\xspace}

%-----------------------------------------------------------------------------------------------------.
% Dynamics

\newcommand{\bMth}{\ensuremath{\bs{M_\theta}}\xspace}
\newcommand{\bCth}{\ensuremath{\bs{C_\theta}}\xspace}
\newcommand{\bGth}{\ensuremath{\bs{G_\theta}}\xspace}

\newcommand{\bin}{\ensuremath{\bs{I}_n}\xspace}
\newcommand{\Ith}{\ensuremath{I(\theta)}\xspace}

\newcommand{\bkp}{\ensuremath{\boldsymbol{K}_p}\xspace}
\newcommand{\bkv}{\ensuremath{\boldsymbol{K}_v}\xspace}

\newcommand{\bQnc}{\ensuremath{\boldsymbol{Q}^{nc}}\xspace}

%-----------------------------------------------------------------------------------------------------.
% Manipulators

\newcommand{\rrs}{\ensuremath{3}-\underline{R}RS\xspace}
\newcommand{\rps}{\ensuremath{3}-R\underline{P}S\xspace}
\newcommand{\upu}{\ensuremath{3}-U\underline{P}U\xspace}
%\newcommand{\map}{\mbox{MaPaMan}\xspace}
%\newcommand{\mapI}{\mbox{MaPaMan-I}\xspace}
%\newcommand{\mapII}{\mbox{MaPaMan-II}\xspace}
\newcommand{\rrr}{\ensuremath{3}-\underline{R}RR\xspace}
\newcommand{\rpr}{\ensuremath{3}-R\underline{P}R\xspace}

%-----------------------------------------------------------------------------------------------------

% Math Symbols

\renewcommand{\iff}{\ensuremath{\mathit{iff}}\xspace}
%\newtheorem{thm}{Theorem}[section]
%\newcommand{\implies}{\ensuremath{\Rightarrow \;}\xspace}
\def\QED{\ensuremath{\rule[0pt]{1.5ex}{1.5ex}}\xspace}
\def\proof{\noindent\hspace{2em}{\em Proof: }}
\def\endproof{\hspace*{\fill}~\QED\par\endtrivlist\unskip}
%\newcommand{\mathe}{\begin{verbatim}Mathematica\end{verbatim}\xspace}
%\newcommand{\define}{\ensuremath{\stackrel{\Delta}{=}}\xspace}
\newcommand{\elim}[1]{\ensuremath{\stackrel{\times #1}{\longrightarrow}}\xspace}

%% Operations
\newcommand{\adj}{\text{adj}}
\newcommand{\trace}{\text{tr}}

%%% Norm
\newcommand{\norm}[1]{\ensuremath{\| #1\|}\xspace}
\newcommand{\normd}[1]{\ensuremath{\| #1\|_d}\xspace}

%%% Partial derivative
\newcommand{\pd}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}\xspace}
\newcommand{\dpd}[2]{\ensuremath{\dfrac{\partial #1}{\partial #2}}\xspace}

%%% Total derivative
\newcommand{\td}[2]{\ensuremath{\frac{d #1}{d #2}}\xspace}
\newcommand{\dtotder}[2]{\ensuremath{\dfrac{d #1}{d #2}}\xspace}

%%% Partial second derivative
\newcommand{\pdd}[2]{\ensuremath{\frac{\partial^2 #1}{\partial #2^2}}\xspace}

%%% Total second derivative
\newcommand{\tdd}[2]{\ensuremath{\frac{d^2 #1}{d #2^2}}\xspace}
\newcommand{\dsecder}[2]{\ensuremath{\dfrac{\partial^2 #1}{\partial #2^2}}\xspace}

%%% Scalar tripple product
\newcommand{\trip}[3]{\ensuremath{\left[#1, #2, #3\right]\xspace}}

%% Rank symbols
%\newcommand{\rank}[1]{\ensuremath{\mathrm{rank}\left(#1\right)}\xspace}

%-----------------------------------------------------------------------------------------------------

% Generic words

\newcommand{\dof}{degree-of-freedom\xspace}
\newcommand{\dofs}{degrees-of-freedom\xspace}
\newcommand{\rb}{rigid-body\xspace}
\newcommand{\rbm}{rigid-body motion\xspace}

%-----------------------------------------------------------------------------------------------------

